Automatically Improving LLM-based Verilog Generation using EDA Tool Feedback

Traditionally, digital hardware designs are written in the Verilog hardware description language (HDL) and debugged manually by engineers. This can be time-consuming and error-prone for complex designs. Large Language Models (LLMs) are emerging as a potential tool to help generate fully functioning HDL code, but most works have focused on generation in the single-shot capacity: i.e., run and evaluate, a process that does not leverage debugging and, as such, does not adequately reflect a realistic development process. In this work, we evaluate the ability of LLMs to leverage feedback from electronic design automation (EDA) tools to fix mistakes in their own generated Verilog. To accomplish this, we present an open-source, highly customizable framework, AutoChip, which combines conversational LLMs with the output from Verilog compilers and simulations to iteratively generate and repair Verilog. To determine the success of these LLMs we leverage the VerilogEval benchmark set. We evaluate four state-of-the-art conversational LLMs, focusing on readily accessible commercial models. EDA tool feedback proved to be consistently more effective than zero-shot prompting only with GPT-4o, the most computationally complex model we evaluated. In the best case, we observed a 5.8% increase in the number of successful designs with a 34.2% decrease in cost over the best zero-shot results. Mixing smaller models with this larger model at the end of the feedback iterations resulted in equally as much success as with GPT-4o using feedback, but incurred 41.9% lower cost (corresponding to an overall decrease in cost over zero-shot by 89.6%).

==> Tables/feedback_tokens.tex <==

\centering
\footnotesize
\caption{\small }
\label{tab:tokens-and-cost}

\resizebox{0.49\linewidth}{!}{
\begin{tblr}{
colspec = c|c|c|ccc|ccc,
row{1-2} = {font=\bfseries},
column{1} = {font=\bfseries}
}
\toprule
\SetCell[r=2]{c}{Feedback} & \SetCell[r=2]{c}{Candidates} & \SetCell[r=2]{c}{LLM} & \SetCell[c=3]{c}{Eval-Machine (\%)} &&& \SetCell[c=3]{c}{Eval-Human (\%)} && \\ \hline
& &  & d=1 & d=5 & d=10 & d=1 & d=5 & d=10 \\ \hline
\midrule %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SetCell[r=4]{c}{Full} & \SetCell[r=2]{c}{$k=1$} & Haiku &  &  &  &  &  &   \\
& & GPT-3.5T &  | &  &  &  &  &   \\ \hline
& \SetCell[r=2]{c}{$k=5$} & Haiku &  &  &  &  &  &   \\
& & GPT-3.5T &  &  &  &  &  &   \\ \hline
\hline %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SetCell[r=8]{c}{Succinct} & \SetCell[r=4]{c}{$k=1$} & Haiku &  &  &  &  &  &  \\
& & GPT-3.5T  &  &  &  &  &  &   \\
& & GPT-4o-Mini &  &  &  &  &  &  \\
& & GPT-4o  &  &  &   &  &  &   \\
\hline
& \SetCell[r=4]{c}{$k=5$} & Haiku  &  &  &   &  &  &   \\
& & GPT-3.5T  &  &  &  &  &  &   \\
& & GPT-4o-Mini &  &  &  &  &  &  \\
& & GPT-4o &  &  &  &  &  &   \\
\bottomrule

\end{tblr}
}


==> Tables/feedback_tokens_ensemble.tex <==

\centering
\footnotesize
\caption{\small }
\label{tab:tokens-and-cost-ensemble}

%\resizebox{\linewidth}{!}{
\begin{tblr}{
colspec = c|c|c|ccc|ccc,
row{1-2} = {font=\bfseries},
column{1} = {font=\bfseries}
}
\toprule
\SetCell[r=2]{c}{Feedback} & \SetCell[r=2]{c}{Candidates} & \SetCell[r=2]{c}{LLM} & \SetCell[c=3]{c}{Eval-Machine (\%)} &&& \SetCell[c=3]{c}{Eval-Human (\%)} && \\ \hline
& &  & d=1 & d=5 & d=10 & d=1 & d=5 & d=10 \\ \hline
\midrule %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SetCell[r=4]{c}{Full} & \SetCell[r=2]{c}{$k=1$} & Haiku &  &  &  &  &  &   \\
& & GPT-3.5T &  &  &  &  &  &   \\ \hline
& \SetCell[r=2]{c}{$k=5$} & Haiku &  &  &  &  &  &   \\
& & GPT-3.5T &  &  &  &  &  &   \\ \hline
\hline %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SetCell[r=8]{c}{Succinct} & \SetCell[r=4]{c}{$k=1$} & Haiku &  &  &  &  &  &  \\
& & GPT-3.5T  &  &  &  &  &  &   \\
& & GPT-4o-Mini &  &  &  &  &  &  \\
& & GPT-4o  &  &  &   &  &  &   \\
\hline
& \SetCell[r=4]{c}{$k=5$} & Haiku  &  &  &   &  &  &   \\
& & GPT-3.5T  &  &  &  &  &  &   \\
& & GPT-4o-Mini &  &  &  &  &  &  \\
& & GPT-4o &  &  &  &  &  &   \\
\bottomrule

\end{tblr}
%}


==> Tables/percentage_results.tex <==

\centering
\footnotesize
\caption{\small Pass@k for k=\{1,5\} (w)ith and (w/o)ithout feedback. For (w) feedback, we use $n$ iterations with either the most recent feedback (succinct) or with context retained from all iterations (full). `+GPT-4$^*$'-- Ensemble using GPT-4 as `big' LLM for addressing errors. %(-): NA, refer to~\Cref{subsec:choice_llm}.
}
\label{tab:results}


\begin{tblr}{
colspec = c|c|c|c|ccc|c|ccc|c|ccc,
row{1-2} = {font=\bfseries},
column{1} = {font=\bfseries}
}
\toprule
\SetCell[r=2]{c}{Feedback} & \SetCell[r=2]{c}{Candidates} & \SetCell[r=2]{c}{LLM} & \SetCell[c=4]{c}{Success (\%)} &&&& \SetCell[c=4]{c}{Simulation Error (\%)} &&&& \SetCell[c=4]{c}{Compilation Error (\%)} &&& \\ \hline
& & & d=0 & d=1 & d=5 & d=10 & d=0 & d=1 & d=5 & d=10 & d=0 & nd1 & d=5 & d=10\\ \hline
\midrule %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SetCell[r=4]{c}{Full} & \SetCell[r=2]{c}{$n=1$} & Haiku & 32.50 & 37.50 & 44.17 & \textbf{47.50} & 36.67 & 46.67 & 54.17 & 50.83 & 30.83 & 15.83 & 1.67 & \textbf{1.67} \\
& & GPT-3.5T & 26.45 & 30.00 & 35.00 & \textbf{37.50} & 40.50 & 50.00 & 55.83 & 57.50 & 33.06 & 20.00 & 9.17 & \textbf{5.00} \\ \hline
& \SetCell[r=2]{c}{$n=5$} & Haiku & 32.83 & 38.58 & 45.35 & \textbf{47.38} & 40.83 & 48.39 & 50.42 & 50.08 & 26.33 & 13.03 & 4.23 & \textbf{2.54} \\
& & GPT-3.5T & 27.27 & 31.17 & 36.00 & \textbf{39.00} & 37.69 & 49.33 & 55.50 & 54.67 & 35.04 & 19.50 & 8.50 & \textbf{6.33} \\ \hline
\midrule %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SetCell[r=6]{c}{Succinct} & \SetCell[r=3]{c}{$n=1$} & Claude 2& 31.67 & 33.33 & 41.23 & \textbf{42.11} & 36.67 & 56.14 & 54.39 & 54.39 & 31.67 & 10.53 & 4.39 & \textbf{3.51} \\
& & GPT-3.5T & 26.67 & 30.25 & 34.45 & \textbf{36.13} & 33.33 & 43.70 & 53.78 & 52.94 & 40.00 & 26.05 & 11.76 & \textbf{10.92} \\
& & GPT-4o & 60.83 & 69.16 & \textbf{81.16} & - & 19.16 & 18.33 & 12.5 & - & 20.0 & 12.5 & 7.3 & - \\
\hline
& \SetCell[r=3]{c}{$n=5$} & Haiku & 32.50 & 36.71 & 42.48 & 44.23 & 38.67 & 48.95 & 51.57 & 50.70 & 28.83 & 14.34 & 5.94 & 5.07 \\
& & GPT-3.5T & 28.00 & 30.47 & 34.51 & 36.36 & 35.67 & 48.82 & 56.06 & 55.39 & 38.33 & 20.71 & 9.43 & \textbf{8.25} \\
& & GPT-4o & 60.83 & 69.16 & \textbf{81.16} & - & 19.16 & 18.33 & 12.5 & - & 20.0 & 12.5 & 7.3 & - \\
\hline
\bottomrule

\end{tblr}



==> Tables/zero_shot_tokens.tex <==
\centering
\footnotesize
\caption{}
\label{tab:zero-shot-tokens}
%\resizebox{\linewidth}{!}{
\begin{tblr}{
colspec = c|cccccc|cccccc,
row{1-2} = {font=\bfseries},
column{1} = {font=\bfseries}
}
\toprule
\SetCell[r=2]{c}{Model} & \SetCell[c=6]{c}{Eval-Machine (\%)} &&&&&& \SetCell[c=6]{c}{Eval-Human (\%)} &&&&& \\ \hline
& k=1 & k=5 & k=10 & k=25 & k=30 & k=55 & k=1 & k=5 & k=10 & k=25 & k=30 & k=55 \\ \hline
\midrule %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Haiku & 69.9 & 79.0 & 83.2 & 83.9 & 83.9 & 84.6 & 51.9 & 62.2 & 67.3 & 69.2 & 70.5 & 73.1 \\
GPT-3.5T & 53.1 & 79.7 & 78.3 & 81.8 & 87.4 & 85.3 & 31.4 & 49.4 & 56.4 & 63.5 & 61.5 & 66.0  \\
GPT-4o-Mini & 62.2 & 72.0 & 72.7 & 76.9 & 76.2 & 76.2 & 51.9 & 59.6 & 64.1 & 67.9 & 66.7 & 67.9 \\
GPT-4o & 65.7 & 74.1 & 76.2 & 78.3 & 79.7 & 83.2 & 61.5 & 69.9 & 75.0 & 76.9 & 78.2 & 78.2 \\ \hline \hline
VerilogEval* & 46.2 & 67.3 & 73.7 & - & - & - & 28.8 & 45.9 & 52.3 & - & - & -\\
RTLCoder* & 61.2 & 76.5 & 81.8 & - & - & - & 41.6 & 50.1 & 53.4 & - & - & -  \\
\bottomrule

\end{tblr}
%}

==> section/Approach.tex <==
\section{Proposed Method}

==> section/Evaluation.tex <==
\section{Evaluation}

% \begin{table*}
% \footnotesize

% \centering 
% \caption{Problems for evaluation}
% \begin{tabularx}{\textwidth}
% {|m{0.1\textwidth}|m{0.1\textwidth}|m{0.04\textwidth}|X|}
% \hline
% Difficulty & Category & Count & Problem Description \\ \hline
% % Getting Started & Getting Started & 2 & Getting Started, Output Zero \\ \hline
% \multirow{5}{*}{Verilog} & Basics & 8 & Simple/Four wires, Inverter, AND, NOR, XNOR, Declare wires, 7458 chip \\ \cline{2-4}
%  & Vectors & 9 & Vectors, Vectors (  detail), Vector part select, Bitwise operators, Four-input gates, Vector concatenate, Vector reversal 1, Replicate, More replication \\ \cline{2-4}
%  & Module Hierarchy & 9 & Modules, Connect ports by position, Connect ports by name, Three modules, Modules and vectors, Adder 1, Adder 2, Carry-select, Adder-subtractor \\ \cline{2-4}
%  & Procedures & 8 & Always blocks (combinational), Always blocks (clocked), If statement, If statement latches, Case statement, Priority encoder, Priority encoder with casez, Avoiding latches \\ \cline{2-4}
%  & More Features & 7 & Conditional ternary, Reduction operators, Reduction: Wider gates, Combinational for-loop: Vector reversal 2, Combination for-loop: 255-bit count, Generate for-loop: 100-bit adder 2, Generate for-loop: 100-digit BCD adder \\ \hline
% \multirow{4}{*}{Circuits} & Basic & 17 & Wire, GND, NOR, Another, Two gates, More gates, 7420 chip, Truth tables, Two-bit equality, Simple circuits A, B, Combine circuits A, B, Ring or vibrate?, Thermostat, 3-bit count, Gates and vectors, longer vectors \\ \cline{2-4}
% (Combination) & Multiplexers & 5 & 2-to-1 mux, 2-to-1 bus mux, 9-to-1 mux, 256-to-1 mux, 256-to-1 4-bit mux\\ \cline{2-4}
%  & Arithmetic Circuits & 7 & Half adder, Full adder, 3-bit adder, Signed addition overflow, 100-bit binary adder, 4-digit BCD adder \\ \cline{2-4}
%  & K-Map to Circuit & 8 & 3/4-variable, Minimum SOP and POS, K-map, K-map  with a mux \\ \hline
% \multirow{8}{*}{Circuits } & Latches and Flip-Flops & 18 & DFFs, DFF (reset), DFF (reset value), DFF (asynchronous), DFF (byte enable), D Latch, DFF,  DFF+gate, Mux and DFF, DFFs and gates, Circuit from truth table, Detect edge/both edges, Edge capture register, Dual-edge triggered FF \\ \cline{2-4}
% & Counters & 8 & Four-bit binary counter, Decade counter, Decade counter again, Slow decade counter, Counter 1-12, Counter 1000, 4-digit decimal counter, 12-hour clock \\ \cline{2-4}
%  (Sequential)  & Shift Registers & 9 & 4-bit shift register, Left/right rotator, Left/right arithmetic shift by 1 or 8, 5-bit LFSR, 3-bit LFSR, 32-bit LFSR, Shift register, Shift register, 3-input LUT \\ \cline{2-4}
%  & Cellular Automata & 3 & Rule 90, Rule 110, Conways Game of Life 16x16 \\ \cline{2-4}
%  & FSM & 33 & FSM 1 (asynchronous), FSM 1 (synchronous), FSM 2 (asynchronous), FSM 2 (synchronous), Simple state transitions 3, Simple one-hot state transition 3, FSM 3 (asynchronous), FSM 3 (synchronous), Moore FSM, Lemmings 1, Lemmings 2, Lemmings 3, Lemmings 4, One-hot FSM, PS/2 packet parser, PS/2 packet parser and datapath, Serial receiver, Serial receiver and datapath, Serial receiver with parity check, Sequence recognition, Q8: Design Mealy FSM, Q5a: Serial twos complementer (Moore FSM), Q5b: Serial twos complementer (Mealy FSM), Q2a, Q2b, Q3a, Q3b: FSM, Q3c: FSM logic, Q6b: FSM next-state logic, Q6c: FSM one-hot next-state logic, Q6: FSM, Q2a: FSM, Q2b: One-hot FSM equations  \\  \cline{2-4} 
%  & Larger Circuits & 7 & Counter with period 1000, 4-bit shift register and down counter, FSM: Sequence 1101 recognizer, FSM: Enable shift register, FSM: Complete FSM, Complete timer, FSM: One-hot logic equations \\ \hline
% Verify Bugs & Read Simulations \& Find bugs & 5 & Mux2, NAND, Mux4, Add/subtract, Case statement \\ \hline
% \end{tabularx}
% \label{tbl:problems-set-2}
% \end{table*}

















==> section/Fig5.tex <==
\begin{figure}[ht]
\subfloat[Iter 0, Prompt with problem description, vector concatenate. ]{
    \label{fig:vec-prompt}
    \parbox{0.97\columnwidth}{
    \lstinputlisting[language=verilog]{fig5-orig/code1.txt}
    \vspace{-0.5em}
    } 
}

% \hfill%
    \vspace{-1em}% \vspace{-0.3em}
\subfloat[Iter. 0: LLM Response, Simulation Error: 25-of-26 tests fail. ]{
    \label{fig:vec-iteration0}
    \parbox{0.97\columnwidth}{
    \lstinputlisting[language=verilog]{fig5-orig/code2.txt} 
    \vspace{-0.5em}
    }
}
    \vspace{-0.2em}
\subfloat[Iter. 1: LLM Response, Simulation Error: Tests 1-2 pass. 23 tests fail.]{
    \label{fig:vec-iteration1}
    \parbox{0.97\columnwidth}{
    \lstinputlisting[language=verilog]{fig5-orig/code3.txt} 
    \vspace{-0.5em}
    }
}
    \vspace{-0.2em}
\subfloat[Iter. 2: LLM Response, Simulation Error: Tests 1-10 pass and rest  fail.]{
    \label{fig:vec-iteration2}
    \parbox{0.97\columnwidth}{
    \lstinputlisting[language=verilog]{fig5-orig/code4.txt} 
    \vspace{-0.5em}
    }
}
    \vspace{-0.2em}
\subfloat[Iter. 3: LLM Response, Simulation Error: Tests 1-12 pass and rest fail.]{
    \label{fig:vec-iteration3}
    \parbox{0.97\columnwidth}{
    \lstinputlisting[language=verilog]{fig5-orig/code5.txt} 
    \vspace{-0.5em}
    }
}
    \vspace{-0.2em}
\subfloat[Iter. 4: All Tests Pass. Testbench ran successfully.]{
    \label{fig:vec-iteration4}
    \parbox{0.97\columnwidth}{
    \lstinputlisting[language=verilog]{fig5-orig/code6.txt} 
    \vspace{-0.5em}
    }
}

\caption{LLM: GPT-3.5-turbo, vector concat with feedback.\label{fig:vector-iterations}}

\end{figure}

==> section/Fig6.tex <==
\begin{figure}[ht]
\subfloat[Iteration 0, User Prompt, Category 3: FSM serial receiver and data path]{
\label{fig:fsm-prompt}

\parbox{\columnwidth}{
\lstinputlisting[language=verilog]{fig6-orig/code1.sv} \vspace{-0.5em}
}
}
\hfill%
\subfloat[Diff b/w LLM Response from Iter. 0 and  1. Iter. 1, Compile Error: testbench failed to compile, At line 54, `done' is used as an l-value but was declared as a wire at line 6. Wires cannot be used as l-values. At line 60, `done' is used as an l-value but was declared as a wire at line 6.
]{
\label{fig:fsm-iter1}

\parbox{\columnwidth}{
\vspace{-1.2em}
\lstinputlisting[language=diff]{fig6-orig/code2.sv} \vspace{-0.5em}
}
}
\hfill%
\subfloat[Diff b/w LLM response from Iter. 1 and Iter. 2. Iter. 2, Simulation Error: Test 1-7,11-6,20,23-25 passed! 11 fail.
]{
\label{fig:fsm-iter2}

\parbox{\columnwidth}{
\vspace{-1.2em}
\lstinputlisting[language=diff]{fig6-orig/code3.sv} \vspace{-0.5em}
}
}
\hfill%
\subfloat[Diff b/w Iteration 2 and Iteration 3 (All Tests passed!)
]{
\label{fig:fsm-iter3}

\parbox{\columnwidth}{
\vspace{-1.2em}
\lstinputlisting[language=diff]{fig6-orig/code4.sv} \vspace{-0.5em}
}
}
\hfill%

\caption{LLM: GPT-3.5-turbo, FSM serial rx (w) feedback.\label{fig:fsm-iters}}
\end{figure}


==> section/problem_sets.tex <==
\begin{table}
\caption{VerilogEval problems, categorized by HDLBits.}%Problems with a \colorbox{hilight_blue}{blue highlight} are only in the Human evaluation set.~\cite{wong_hdlbits_2017, liu_verilogeval_2023}.} 
\label{tbl:problems-set-2}

\begin{tblr}[
    colspec = 
]


\end{tblr}

\end{table}

% \definecolor{hilight_blue}{RGB}{43,188,255}
% \renewcommand{\arraystretch}{1}

% \vspace{-3mm} 
\scriptsize
\resizebox{\textwidth}{!}{%
\begin{tabular}{|C{1.2cm}|C{1.4cm}|L{12cm}|}
\hline
Category-1 & Category-2 & Problem Description \\ \hline
\multirow{5}{*}{Syntax} & Basics & Simple/Four wires, Inverter, AND, NOR, XNOR, Declare wires, 7458 chip \\ \cline{2-3} 
 & (Vec)tors  & Vectors (detail), Vector part select, Bitwise ops, Four-input gates, Vector concat, reversal 1, Replicate, More replication \\ \cline{2-3} 
 & (Mod)ule (Hier)archy  & Modules, Connect ports by position, Connect ports by name, Three modules, Modules and vectors, Adder 1, Adder 2, Carry-select, Adder-subtractor \\ \cline{2-3} 
 & (Proc)edures  & Always blocks (combinational), Always blocks (clocked), If statement, If statement latches, Case statement, Priority encoder, Priority encoder with cases avoiding latches \\ \cline{2-3} 
 & More Features  & Conditional ternary, Reduction operators, Reduction: Wider gates, Combination for-loop: Vector reversal 2, Combination for-loop: 255-bit count, Generate for-loop: 100-bit adder 2, Generate for-loop: 100-digit BCD adder \\ \hline
\multirow{4}{*}{Comb.} & Basic Gates & Wire, GND, NOR, Another, Two gates, More gates, 7420 chip,   Truth tables, Two-bit equality, Simple circuits A, B, Combine circuits A, B,   Ring or vibrate?, Thermostat, 3-bit count, Gates and vectors, longer vectors \\ \cline{2-3} 
 &  Multiplexer & 2-to-1, 2-to-1 bus MUX, 9-to-1, 256-to-1, 256-to-1 4-bit \\ \cline{2-3} 
 &  Arithmetic & Half add, Full add, 3-bit adder, Signed addition overflow,  100-bit binary adder, 4-digit BCD adder \\ \hline 
 &  K-maps & 3/4-variable, Minimum SOP and POS, K-map, K-map with a mux \\ \cline{2-3} 
 \multirow{6}{*}{Sequential} & Latch/FFs & DFFs, DFF (reset), DFF (reset value), DFF (asynch.), DFF (byte   enable), D Latch, DFF, DFF+gate, Mux and DFF, DFFs and gates, Circuit from   truth table, Detect edge/both edges, Edge capture register, Dual-edge   triggered FF \\ \cline{2-3} 
 &  Counters & Four-bit, Decade,   Slow decade counter, Counter 1-12, Counter 1000, 4-digit decimal counter,  12-hour clock \\ \cline{2-3} 
 &  Shift Regs & 4-bit shift reg, Left/right rotate, Left/right arithmetic shift by 1/8, 5-bit/3-bit/32-bit LFSR,  3-input LUT \\ \cline{2-3} 
 &  C Automata & Rule 90, Rule 110, Conway Game of Life 16x16 \\ \cline{2-3} 
 &  FSM & FSM 1 (asynch.), FSM 1 (synch.), FSM 2 (asynch.), FSM 2 (synch.), Simple transitions 3, Simple one-hot state transition 3, FSM 3 (asynch.), FSM 3 (synch.), Moore, One-hot, PS/2 packet parser, PS/2 packet parser and datapath, Serial receiver, Serial receiver and datapath, Serial receiver with parity check, Sequence recognizer, Q8: Mealy FSM, Q5a: Serial twos complementer (Moore), Q5b: Serial twos complementer (Mealy), Q2a, Q2b, Q3a, Q3b: FSM, Q3c: FSM logic, Q6b: FSM next-state logic, Q6c: FSM one-hot next-state logic, Q6: FSM, Q2a: FSM, Q2b: One-hot FSM \\ \cline{2-3} 
 &  Larger Circuits & Counter with period 1000, 4-bit shift register and down counter, FSM: 1101 recognizer, Enable shift register, Complete FSM, timer, one-hot logic \\ \hline
Fix Bugs &  & Mux2, NAND, Mux4, Add/subtract, Case statement \\ \hline
Write Test &   & Clock, T flip-flop \\ \hline
\end{tabular}%
}
\vspace{-3mm}
